In Defense of Online Models for Video Instance Segmentation

In recent years, video instance segmentation (VIS) has been largely advanced by offline models, while online models gradually attracted less attention possibly due to their inferior performance. However, online methods have their inherent advantage in handling long video sequences and ongoing videos while offline models fail due to the limit of computational resources. Therefore, it would be highly desirable if online models can achieve comparable or even better performance than offline models. By dissecting current online models and offline models, we demonstrate that the main cause of the performance gap is the error-prone association between frames caused by the similar appearance among different instances in the feature space. Observing this, we propose an online framework based on contrastive learning that is able to learn more discriminative instance embeddings for association and fully exploit history information for stability. Despite its simplicity, our method outperforms all online and offline methods on three benchmarks. Specifically, we achieve 49.5 AP on YouTube-VIS 2019, a significant improvement of 13.2 AP and 2.1 AP over the prior online and offline art, respectively. Moreover, we achieve 30.2 AP on OVIS, a more challenging dataset with significant crowding and occlusions, surpassing the prior art by 14.8 AP. The proposed method won first place in the video instance segmentation track of the 4th Large-scale Video Object Segmentation Challenge (CVPR2022). We hope the simplicity and effectiveness of our method, as well as our insight into current methods, could shed light on the exploration of VIS models.

==> 01-intro-1.tex <==
Video instance segmentation (VIS) aims at detecting, segmenting, and tracking object instances simultaneously in a given video. It has attracted considerable attention after first defined in 2019 due to the huge challenge it faces and its wide applications in video understanding, video editing, autonomous driving, augmented reality, etc. Current VIS methods can be categorized as online or offline methods. Online methods take as input a video frame by frame, detecting and segmenting objects per frame while tracking instances and optimizing results across frames. Offline methods, in contrast, take the whole video as input and generally generate the instance sequence of the entire video with a single step.

Despite high performance, the requirement of full videos limits the application scenarios of offline models, especially for scenarios involving long video sequences (that are very common in daily life) and ongoing videos (e.g., in the task of autonomous driving, augmented reality, etc.) However, online models are usually inferior to the contemporaneous offline models by over 10 mAP, which is a huge drawback. Previously, little work tries to explain the performance gap between these two paradigms, or gives insight into the high performance of the offline paradigm. A common attempt of the latter is made from the inherent advantages of offline models being able to skip the error-accumulating tracking/matching steps and utilize the richer information provided by multiple frames to improve instance segmentation, which is also the motivation of most previous work in offline models. However, is that really the case, especially for the current offline methods? What's the main problem causing the poor performance of current online models? Can online models have performance comparable to, or even better than, SOTA offline ones?

To deeply understand the performance of both online and offline models, we first analyze in detail several SOTA methods in two datasets with different difficulty levels. The key findings are that, firstly, multiple frames do provide more information compared with a single image for instance segmentation, but in the meantime, they also cause extra noises that are very hard to model due to the high uncertainty. The noises are small and easy to eliminate when handing very short videos with few occlusions, simple motions, and smooth changes in illumination and object shapes. However, they become hard to handle when the video becomes complex, causing the segmentation performance to drop drastically. By contrast, segmentation per frame is much more robust. What’s more, when providing ground-truth instance id, the performance of current SOTA offline models, which only depend on the quality of estimated segmentation masks, is much higher when clip size is set to one (i.e., doing per-frame segmentation), and drops when clip size becomes larger (i.e., doing per-clip/video segmentation). Briefly, although in theory, per-clip segmentation has its inherent advantage to using multiple frames, it still requires further exploration, especially in how to utilize information in multiple frames and how to handle the noises. On the other hand, per-frame segmentation of online VIS methods enjoys the latest progress in the field of image segmentation. It is accurate, fast, robust, and is not the reason for the poor performance of online methods.

% From the perspective of instance segmentation, \textbf{firstly}, multiple frames theoretically provide more information compared with a single image, but in practice, they also cause extra noises that are very hard to model due to the high uncertainty. The noises are small and easy to eliminate when handing very short videos with few occlusions, simple motions, and smooth changes in illumination and object shapes. However, they become hard to handle when the video becomes complex, causing the segmentation performance to drop drastically. By contrast, segmentation per frame is much more robust. \textbf{Secondly}, when providing ground-truth instance id, the performance of current SOTA offline models, which only depend on the quality of estimated segmentation masks, is much higher when clip size is set to one (i.e., it is actually doing per-frame segmentation), and drops when clip size becomes larger (i.e., doing per-clip/video segmentation). For current offline methods, when all models have perfect association modules, using multiple frames actually degrades performance. \textbf{To sum up}, although in theory, per-clip segmentation has its inherent advantage to using multiple frames, it still requires further exploration, especially in how to utilize information in multiple frames and how to handle the noises. On the other hand, per-frame segmentation is accurate, fast, robust, and is not the reason for the poor performance of online methods.

Secondly, direct generating instance sequences of the entire video avoids the use of hand-designed association modules, which works well on simple cases in the YouTube-VIS dataset. We demonstrate that it is the main reason causing the performance gap between the current online and offline paradigms. However, this black-box association process done within offline models is very sensitive and will get worse rapidly when the video becomes complex. In addition, when handling longer videos, e.g. videos in the real world or from OVIS dataset, offline methods require splitting the input video into clips to avoid exceeding computational limits, and thus hand-designed clip matching is still inevitable, which will further decrease the overall performance. In general, matching/tracking is still one of the key problems of VIS, both for online models, since it causes the performance gap, and for offline models, since it is still inevitable and greatly degrades the performance when handling complex cases.

% From the perspective of association, \textbf{firstly}, a huge advantage to direct generating instance sequences of the entire video is its ability to avoid the use of hand-designed association modules. It works well on simple cases in the YouTube-VIS dataset. We demonstrate that it is the main reason causing the performance gap between the current online and offline paradigms. \textbf{However}, this black-box association process done within offline models is very sensitive and will get worse rapidly when the video becomes complex. \textbf{In addition}, when handling longer videos, e.g. videos in the real world or from OVIS dataset, offline methods require splitting the input video into clips to avoid exceeding computational limits, and thus hand-designed clip matching is still inevitable, which will further decrease the overall performance. \textbf{To sum up}, matching/tracking is the main reasoning of the performance gap, and it is still inevitable and of great importance for offline models.

To improve the matching performance and thus bridge the performance gap, we propose XXX. The key idea is to ensure, in the embedding space, the similarity of the same instance across frames and the difference of different instances in all frames, even instances that belong to the same category and have very similar appearances. It provides instance features more discriminative and with better temporal consistency, which guarantees more accurate association results. In addition, to solve the problem caused by occlusions and crowded scenes, we formulate the problem of positive and negative samples selection as an Optimal Transport problem in Optimization Theory. Specifically, xxx. During Inference, by using one-to-many temporal-weighted softmax, we utilize the learned prior information of the embedding to re-identify missing instances caused by occlusions and to enforce the consistency and integrality of associations. 

==> 01-intro-2.tex <==
Video instance segmentation aims at detecting, segmenting, and tracking object instances simultaneously in a given video. It attracted considerable attention after first defined~\cite{MaskTrackRCNN} in 2019 due to the huge challenge and the wide applications in video understanding, video editing, autonomous driving, augmented reality, etc. Current VIS methods can be categorized as online or offline methods. Online methods~\cite{MaskTrackRCNN,sipmask,compfeat,STMask,CrossVIS,PCAN} take as input a video frame by frame, detecting and segmenting objects per frame while tracking instances and optimizing results across frames. Offline methods~\cite{MaskProp,ProposeReduce,STEmSEG,VisTR,IFC,seqformer}, in contrast, take the whole video as input and generate the instance sequence of the entire video with a single step.


\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{Figs/motivation.pdf}
	\caption{\textbf{Oracle experiments on SOTA offline methods: } We analyze current VIS methods and visualize some results here. More results can be found in Sec.~\ref{sec:VIS-Analysis}. `YTVIS' is short for YouTube-VIS 2019. `Frame' and `clip' stand for frame oracle and clip oracle experiments, respectively. For frame oracles, we provide the ground-truth instance ID both within each clip and between adjacent clips. Thus the performance only depends on the quality of the estimated segmentation masks. For clip oracles, we only provide the ground-truth instance ID between adjacent clips, and the method is required to do association within the clips by itself. Therefore the gaps between frame oracles and clip oracles show the effect of the black-box association done within current offline models. When clip length is 1, the method is doing per-frame segmentation.}
	\label{fig:motivation}
\end{figure}


Despite high performance, the requirement of full videos limits the application scenarios of offline models, especially for scenarios involving long video sequences (videos exceed 50 frames on GPU of 32G RAM~\cite{seqformer}) and ongoing videos (\eg, videos in autonomous driving and augmented reality). However, online models are usually inferior to the contemporaneous offline models by over 10 AP, which is a huge drawback. Previously, little work tries to explain the performance gap between these two paradigms, or gives insight into the high performance of the offline paradigm. A common attempt of the latter is made from the inherent advantages of offline models being able to skip the error-accumulating tracking/matching steps~\cite{ProposeReduce} and utilize the richer information provided by multiple frames to improve segmentation~\cite{IFC,STEmSEG,seqformer}. However, does that really explain the high performance of current offline methods? What's the main problem causing the poor performance of online models? Can online models achieve performance comparable to, or even better than, SOTA offline ones?

To deeply understand the performance of both online and offline models, we analyze in detail three SOTA methods (offline: IFC~\cite{IFC} and SeqFormer~\cite{seqformer}, online: CrossVIS~\cite{CrossVIS}) on two datasets (YouTube-VIS~\cite{MaskTrackRCNN} and OVIS~\cite{ovis}) that have different difficulty levels. `Simple video' refers to the video in YouTube-VIS. These videos are much shorter and only contain very slight occlusions, simple motions, and smooth changes in illumination and object shapes. `Complex video' refers to the video in OVIS. Please see Sec.~\ref{sec:dataset} for details. The results (Fig.~\ref{fig:motivation}) of our oracle experiments give us a deep understanding of current SOTA methods:


From the perspective of instance segmentation, per-clip segmentation doesn't outperform per-frame segmentation a lot in mask quality, and mask quality is also not the reason for the poor performance of online methods: CrossVIS even outperforms its contemporaneous work (\ie IFC) in frame oracle experiments on both datasets (results in Table~\ref{table:crossvis_IFC}). What's more, per-clip segmentation of current SOTA methods is not effective and robust. Multiple frames do provide more information and improve the mask quality by 3.7 AP for IFC on YouTube-VIS (Fig.~\ref{fig:motivation}). But it only works for some cases: per-clip segmentation doesn't improve the performance of SeqFormer a lot. In addition, when testing on more challenging datasets like OVIS, segmentation on multiple frames even degrades the performance by 1.8 and 2.2 AP on IFC and SeqFormer respectively when clip size becomes longer.
Although in theory, per-clip segmentation has its inherent advantage to using multiple frames, it still requires further exploration, especially in how to utilize information in multiple frames and how to handle complex motion patterns, occlusion, and object deformation. Currently, we don't see an obvious gap between the mask qualities of per-clip and per-frame segmentation. 

From the perspective of association, a huge advantage of the offline methods is their ability to avoid the use of hand-designed association modules. It works well on simple cases of the YouTube-VIS dataset. We demonstrate that it is the main reason causing the performance gap between the current online and offline paradigms. However, this black-box association process done within offline models also gets worse rapidly when the video becomes complex (degrades the performance of IFC by 12.3 AP and SeqFormer by 20.9 AP on OVIS). In addition, when handling longer videos, \eg videos in the real world or from OVIS dataset, offline methods require splitting the input video into clips to avoid exceeding computational limits, and thus hand-designed clip matching is still inevitable, which will further decrease the overall performance. To sum up, matching/association is the main reasoning for the performance gap, and it is still inevitable and of great importance for offline models.

To improve the matching performance and thus bridge the performance gap, we propose a framework \textbf{I}n \textbf{D}efense of \textbf{O}n\textbf{L}ine model for video instance segmentation, termed IDOL. The key idea is to ensure, in the embedding space, the similarity of the same instance across frames and the difference of different instances in all frames, even for instances that belong to the same category and have similar appearances. It provides more discriminative instance features with better temporal consistency, which guarantees more accurate association results.
However, previous method~\cite{QDTrack} selects positive and negative samples by a hand-craft setting, introducing false positives in occlusions and crowded scenes, thus impairing contrastive learning. To address it, we formulate the problem of sample selection as an Optimal Transport problem in Optimization Theory, which reduces false positives and further improves the quality of the embedding.
During inference, by using one-to-many temporally weighted softmax, we utilize the learned prior of the embedding to re-identify missing instances caused by occlusions and to enforce the consistency and integrality of associations. 

Our thorough analysis gives us a deep understanding of current online and offline VIS methods. Based on our observation, we bridge the performance gap from the perspective of feature embeddings and propose IDOL. We conduct extensive experiments on YouTube-VIS 2019, YouTube-VIS 2021, and OVIS datasets. Despite its simplicity, our method sets a new state-of-the-art achieving 61.5 AP, 56.1 AP, and 42.6 AP on the validation set of these three benchmarks, respectively. More importantly, compared with previous online methods, we achieve a consistent improvement ranging from 10.6 AP to 14.7 AP on these datasets. We even surpass the previous SOTA offline method by up to 2.2 AP. We believe the simplicity and effectiveness of our method shall benefit further research. In addition, our thorough analysis provides insights for current methods and suggests useful directions for future work in both online and offline VIS.

==> 01-intro-sketch.tex <==
\noindent From the perspective of mask quality: (paragraph 3)
\begin{itemize}
\item Multiple frames segmentation doesn't improve a lot compared with single frame segmentation.
\item Per-clip segmentation gets worse rapidly when videos become complex (AP drops from 51.8 to 22.8 for IFC and from 57.0 to 29.8 for SeqFormer). By contrast, per-frame segmentation is more robust (? vs ?).
\item Multiple frames do provide more information compared with a single image and thus improve the mask quality by up to 3.7 for IFC and 1.3 for SeqFormer. But it only works for simple videos. When testing on OVIS, multiple frames segmentation only improve the mask quality by at most 1.3 for IFC and 0.3 for SeqFormer. What's more, the improvement is less obvious in practice, even for simple videos, due to the association problem mentioned in next paragraph.
\item (conclusion) Mask quality is not the reason causing performance gap.
\item (conclusion) Although in theory, per-clip segmentation has its inherent advantage to using multiple frames, it still requires further exploration, especially in how to utilize information in multiple frames and how to handle complex motion pattern, occlusion, and object deformation.
\end{itemize}

\noindent From the perspective of association quality: (paragraph 4)
\begin{itemize}
\item Offline model is able to avoid the use of hand-designed association modules, which works well on simple cases in the YouTube-VIS dataset. We demonstrate that it is the main reason causing the performance gap.
\item Association quality of the black-box association in offline model also get worse rapidly when videos become complex
\item Hand-designed association module is actually inevitable for longer videos, and it will further decrease the overall performance of offline models.
\item (conclusion) Hand-designed association module is the main reason of the performance gap, and it still inevitable for offline models. 
\end{itemize}
